FastDeepIoT: Towards Understanding and Optimizing Neural Network Execution Time on Mobile and Embedded Devices

Deep neural networks show great potential as solutions to many sensing application problems, but their excessive resource demand slows down execution time, pausing a serious impediment to deployment on low-end devices. To address this challenge, recent literature focused on compressing neural network size to improve performance. We show that changing neural network size does not proportionally affect performance attributes of interest, such as execution time. Rather, extreme run-time nonlinearities exist over the network configuration space. Hence, we propose a novel framework, called FastDeepIoT, that uncovers the non-linear relation between neural network structure and execution time, then exploits that understanding to find network configurations that significantly improve the trade-off between execution time and accuracy on mobile and embedded devices. FastDeepIoT makes two key contributions. First, FastDeepIoT automatically learns an accurate and highly interpretable execution time model for deep neural networks on the target device. This is done without prior knowledge of either the hardware specifications or the detailed implementation of the used deep learning library. Second, FastDeepIoT informs a compression algorithm how to minimize execution time on the profiled device without impacting accuracy. We evaluate FastDeepIoT using three different sensing-related tasks on two mobile devices: Nexus 5 and Galaxy Nexus. FastDeepIoT further reduces the neural network execution time by $48\%$ to $78\%$ and energy consumption by $37\%$ to $69\%$ compared with the state-of-the-art compression algorithms.

==> Discussion.tex <==
\vspace{-0.3cm}
\section{Discussion}~\label{sec:discussion}
%As the first step towards understanding deep neural network execution time on mobile and embedded devices, 
In this paper,  we described a system that automatically builds execution time models for neural network components then uses those to better compress neural networks for execution on mobile devices without loss of accuracy. We test the system on two hardware platforms showing improved execution time and energy consumption. In order to fully understand the execution time behaviours of neural networks on all commonly used hardware, there is still a long way to go. More profiling results with the different choices of hardware, OS versions, and deep learning libraries are needed. These choices can have a huge effect on the execution time behaviours. We will open our profiling results to facilitate future research on modelling deep learning execution time.

Currently, FastDeepIoT can only support deep learning structure compression algorithms. In order to make FastDeepIoT support other deep learning compression methods, such as parameter quantization and pruning~\cite{han2015deep},
%, for reducing model execution time proper. 
future research on modelling the execution time of deep neural networks with quantized or sparse matrices are needed.

%In addition, although FastDeepIoT can save more energy than all other baseline algorithms in almost all our evaluation cases, we still require an interpretable modeling on deep learning energy consumptions. As illustrated in our evaluation results, Figure~\ref{fig:CIFAR10_acc_energy_n5},~\ref{fig:CIFAR10_acc_energy_gn},~\ref{fig:imageNet_acc_energy_n5},~\ref{fig:imageNet_acc_energy_gn},~\ref{fig:HHAR_acc_energy_n5}, and~\ref{fig:HHAR_acc_energy_gn}, execution time and energy consumption of deep learning components clearly follow different modeling. Modelling and understanding the deep learning energy consumption can help us to design energy efficient deep learning structures.

In addition, our execution time model explores some new modalities for neural network model compression. As shown in Section~\ref{sec:exp_HHAR}, the setup overhead of recurrent layers imposes an execution time lower bound on compression. Therefore, the recurrent neural network steps can be new modality to compress for speeding up recurrent layers.
